Repeated Sales with Heterogeneous Buyer Sophistication

This paper considers behavior-based price discrimination in the repeated sale of a non-durable good to a single long-lived buyer, by a seller without commitment power. We assume that there is a mixed population of forward-looking ``sophisticated'' buyers and myopic ``naive'' buyers. We investigate the impact of these dynamics on the seller's ability to learn about the buyer and exploit this learning for revenue. We obtain conclusions that differ dramatically with the time horizon of the interactions. To understand short time horizons, we analyze a two-period model, and find that the strategic demand reduction observed with fully sophisticated buyers is robust to the introduction of naive types. In fact, despite the inability of naive buyers to game the pricing algorithm, their introduction can further harm the seller's revenue, due to more intense demand reduction overall. For long horizons, we consider an infinite-horizon model with time discounting. We find that the extreme demand reduction predicted by previous work does not survive the introduction of naive buyers. Instead, we observe equilibria where the seller learns meaningfully despite the sophisticated buyers' demand reduction. We prove that for a natural family of such equilibria, the seller's revenue is not just high, but approximates the revenue attainable with commitment power, even when the fraction of naive types is vanishingly small.

==> revenueanalysis.tex <==


\subsection{Proof of the Main Result}
\label{sec:rev}

In this section, we focus on proving the paper's main result. In particular, we demonstrate that the revenue of 
 a sophisticated-focused continuation is increasing in the level of sophistication. In addition, naive-focused continuation is only possible for very high thresholds $t$ as $\mu$ approaches  $1$. Thus, when $\mu$ is sufficiently high, sophisticated-focused equilibria dominate, which implies that the revenue increases with the degree of sophistication. 
First, we prove that if we fix $t$ and increase $\mu$, the unique $p_1$ that implements $t$ must increase.  The full proof is in Appendix~\ref{app:cor:p1growth}.


\begin{lemma}\label{cor:p1growth}
Assume threshold $t$ can be implemented with first-round price $p_1$  at sophistication level $\mu$. Then $p_1$ is continuous, strictly increasing, and differentiable wrt $\mu$. 
\end{lemma}
The results of the previous section imply that if the seller's optimal prices induce sophisticated-focused continuations and that the seller has more and more such continuations to choose from. We will now show show that the seller's revenue in sophisticated-focused continuations increases.
In particular, we fix a threshold $t$, and consider implementing $t$ with higher and higher values of $\mu$. We will show that the seller's revenue improves. Formally:

\begin{lemma}\label{lem:trev}
    Fix any threshold $t$, and let $\mu$ be such that $t$ is implementable in a sophisticated-focused continuation.
    The revenue of the equilibrium is continuous and strictly increasing in $[\mu,1]$.
 \end{lemma}

Despite the relatively simple structure of sophisticated-focused continuations, Lemma~\ref{lem:trev} is not a foregone conclusion.
As we will prove in Section~\ref{sec:whytho}, sophisticated buyers yield less revenue than naive buyers: increasing the population sophistication causes a first-order revenue {\em loss}.
The key insight is a reamortization of the seller's revenue, that allows us to charge the naive buyers' second-round revenue to the sellers.
This allows us to properly quantify the countervailing revenue {\em gains} from the way the prices change with $\mu$.
\begin{proof}
%Let $p_1,p_2^\rej $

The seller's revenue for implementing $t$ can be decomposed as follows:
\begin{align*}
\Rev_1&=R(p_1)(1-\mu) + p_1(1-F(t))\mu\\
\Rev_2^\acc&=\big(\mu(1-F(t))+(1-\mu)(1-F(p_1)\big)R^\acc(t)\\
\Rev_2^\rej&=\big(\mu(F(t))+(1-\mu)(F(p_1)\big)\mathbb E[R^\rej(p_2^\rej)].
\end{align*}

From the characterization of Lemma~\ref{lem:plph}, we know that $p^\rej_2$ is a randomized price supported on two prices $p_L<p_1$ and $p_1\leq p_H=p^*_{\leq t}$ such that $\mathbb E[R^\rej(p_2^\rej)]=R^\rej(p_L)=R^\rej(p^*_{\leq t})$. Hence we may rewrite $\Rev_2^\rej$ to obtain the following reamortization:
$$
\Rev_2^\rej=\mu F(t) R^\rej(p^*_{\leq t})=\mu (F(t)-F(p^*_{\leq t})) p^*_{\leq t} 
$$
Similarly, $\Rev_2^\acc$ can be simplified to obtain
$
\Rev_2^\acc=t(1-F(t)).
$
Thus the total revenue is given by:
\begin{align*}
\Rev&=\Rev_1+\Rev_2^\rej+\Rev_2^\acc\\
&=  (1-\mu)R(p_1)+\mu \big(p_1(1-F(t))+p^*_{\leq t}(F(t)-F(p^*_{\leq t}))\big) +(1-F(t))t\\
&=  R(p_1)+\mu \big(p_1(1-F(t))+p^*_{\leq t}(F(t)-F(p^*_{\leq t}))-(1-F(p_1))p_1\big) +(1-F(t))t
\\
&=  R(p_1)+\mu \big(p^*_{\leq t}(F(t)-F(p^*_{\leq t}))-(F(t)-F(p_1))p_1\big) +(1-F(t))t.
\end{align*}
For a fixed $\mu$ and $t$ admitting sophisticated-focused implementation, the choice of $p_1$ is unique, and moreover from Corollary~\ref{cor:growth}, $p_1$ is continuous in $\mu$, thus, $\Rev$ is also continuous in $\mu$.   
Moreover, $p_1$ is differentiable, and strictly increasing in $\mu$. Letting $p_1'>0$ denote the derivative of this unique $p_1$ with respect to $\mu$,  we may write the derivative of the revenue with respect to $\mu$ as:
\begin{align*}
    (1-F(p_1))p'_1-p_1f(p_1)p'_1 +(F(t)-F(p^*_{\leq t}))p^*_{\leq t}-(F(t)-F(p_1))p_1  \\-\mu((F(t)-F(p_1))p'_1-p_1f(p_1)p_1').
    \end{align*}

    
Since $F_{\leq t}$ is strictly regular, it must be that $p_{\leq t}^*$ is the unique maximizer of $R_{\leq t}$. Hence:
$$(F(t)-F(p^*_{\leq t}))p^*_{\leq t}=R_{\leq t}(p^*_{\leq t})F(t) > R_{\leq t}(p_1)F(t)= (F(t)-F(p))p_1. $$
Thus, we can lower bound the derivative of the revenue as:
\begin{align*}
    &(1-F(p_1))p'_1- p_1f(p_1)p'_1-\mu(F(t)-F(p_1))p'_1+\mu p_1f(p_1)p'_1\\
    &\geq (1-\mu) (1-F(p_1))p'_1- p_1f(p_1)p'_1+\mu p_1f(p_1)p'_1\\
    &= (1-\mu) (1-F(p_1))p'_1 -(1-\mu)p_1f(p)p'_1\\
    &= (1-\mu)( (1-F(p_1))p'_1- p_1f(p)p'_1)\\
    &= (1-\mu)R'(p_1).
    \end{align*}
where the inequality follows from the fact that 
$\mu (1-F(p_1))p'_1 \geq \mu (F(t)-F(p_1))p'_1 $. Finally, we argue that $R'(p_1)>0$ or equivalently $R(p_1)$ increases with $\mu$: from Lemma~\ref{cor:p1growth} we know that $p_1$ increases with $\mu$. 
Lemma~\ref{lem:ordering} implies that $p_1=\mathbb E[p_2^\rej]<p^*$, and hence $R'(p_1)>0$.
\end{proof}

Finally, we show that not only is the revenue increasing for sophisticated-focused implementations in $\mu$, but also, after a certain threshold, the best sophisticated-focused implementation dominates the best naive-focused implementation with respect to revenue. As $\mu$ increases, every naive-focused implementation requires very high values of $t$ --- so high that almost no buyers accept in round $1$.
The full proof is in Appendix~\ref{app:highmblue}.

\begin{lemma}\label{highmublue}
    There exists some $\hat\mu<1$, such that for all $\mu\in[\hat\mu,1]$ the equilibrium is sophisticated-focused.
\end{lemma}

We will use Lemma~\ref{highmublue} to show our main result shortly.
Before proceeding, though, we note that along the way, we have proved that PBE with mixed strategies on-path are necessary.

\begin{corollary}
There exists some $\hat \mu<1$ such that pure strategy equilibrium does not exist, and such that mixed strategy equilibrium mixes on the equilibrium path.
\end{corollary}
\begin{proof}
    Lemma~\ref{highmublue} implies that there is a $\hat\mu<1$ such that the seller's optimal price $p_1^*$ induces a sophisticated-focused implementation. Lemma~\ref{lem:unique} implies that $p_1^*$ does not admit a naive-focused implentation.
    Hence, if the seller is not allowed to mix prices, $p_1^*$ would not admit a solution to the buyer's indifference equation, by Lemma~\ref{lem:plph}.
    By that same lemma, the seller does choose to mix prices if they are allowed and hence mixes on the equilibrium path of play.
\end{proof}




We can now combine all the pieces to prove our main result.

\begin{proof}[Proof of Theorem~\ref{thm:rev}]
Fixing $\mu$, choice of $p_1$ for the seller must induce some continuation, by Lemma~\ref{lem:p1implement}. 
%By Lemmas~\ref{lem:unique} and~\ref{lem:p1uniquet} , whether the continuation is sophisticated-focused or naive-focused is completely determined by $p_1$ and $\mu$. 
Furthermore, by Lemma~\ref{lem:p1uniquet}, if $p_1$ admits a sophisticated-focused implementation, it does not also admit a naive-focused implementation. Furthermore, $p_1$'s sophisticated-focused implementation is unique. Hence, if the seller picks a sophisticated-focused continuation in equilibrium, it must be that the resulting threshold $t$ is revenue-optimal among all $t$ which admit sophisticated-focused implementations. Moreover, Lemma~\ref{highmublue} implies that for sufficiently high $\mu$, the equilibrium must be sophisticated-focused.

We now analyze the seller's revenue as $\mu$ increases. By Corollary~\ref{cor:growth}, the set of thresholds $t$ with sophisticated-focused implementations only grows with $\mu$. Moreover, for any fixed threshold, Lemma~\ref{lem:trev} implies that the seller's revenue in the unique implementation grows. Hence, the seller chooses from more options, each of which yields more revenue as $\mu$ increases, proving the result.
\end{proof}
